Introducing emotions in the reasoning cycle ofnormative aware agents

Human relationships are complex processes that often involve following certain rules that regulate interactions and/or expected outcomes. These rules may be imposed by an authority or established by society. In multi-agent systems, normative systems have extensively addressed aspects such as norm synthesis, norm conflict detection, as well as norm emergence. However, if human behaviour is to be adequately simulated, not only normative aspects but also emotional aspects have to be taken into account. In this paper, we propose a Jason agent architecture that incorporates norms and emotions in its reasoning process to determine which plan (actions) to execute. The proposal is evaluated through a scenario based on a social network, which allows us to analyse the benefits of using emotional normative agents to achieve simulations closer to real human world.

==> 0_images.tex <==
%TODO: Hay que explicar el contenido de las fotos o quitarlas si no son útiles, están comentadas.
\iffalse
\begin{figure}[ht]
\centering
\includegraphics[width=\textwidth]{agent_architecture_simplified.png}
\caption{Simplified normative emotional agent architecture. Derived from \cite{argente2020normative}}
\label{fig:agent_architecture_simplified}
\end{figure}

\begin{figure}[ht]
\centering
\begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{relation1.png}
         \caption{Relation 1: Emotions are considered in the normative reasoning process}
         \label{fig:relation1}
     \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{relation2.png}
         \caption{Relation 2: Norm violation/compliance generates emotions}
         \label{fig:relation2}
     \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{relation3.png}
         \caption{Relation 3: Emotion enables compliance with social norms}
         \label{fig:relation3}
     \end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{relation4.png}
         \caption{Relation 4: Emotion helps internalizing private norms}
         \label{fig:relation4}
     \end{subfigure}
\caption{Architectural representation of how the relations between norms and emotions should be represented. Derived from \cite{argente2020normative}}
\label{fig:norm_emotions_architectural_representation}
\end{figure}
\fi 

==> dropped_content.tex <==
% ANTIGUO ESCENARIO
\begin{comment}
En esta red social los agentes podrán interactuar entre ellos, publicando mensajes sobre una serie de temáticas reducidas, algunas de ellas permitidas y aceptadas por la sociedad, mientras que otras de ellas estarán prohibidas y por tanto repudiadas por los miembros de la red. Cuando un agente publique sobre un tema aceptado, el resto de la sociedad demostrará su aceptación, lo que provocará que el estado afectivo de todos los agentes, tanto emisores como receptores, tienda a ser positivo. En contraposición, cuando un agente publique acerca de un tema prohibido, los agentes le demostrarán su rechazo, lo que provocará nuevamente un cambio en el estado emocional de todos los agentes que tenderá a la negatividad.

Para representar este escenario, se ha dispuesto de una red de 5 agentes normativo emocionales. La selección de temas acerca de los que los agentes pueden hablar en este escenario son de carácter deportivo: tenis, fútbol o baloncesto. Para representar la personalidad de los agentes se utiliza el modelo OCEAN, mientras que para representar su estado afectivo se utiliza el modelo PAD.


\begin{algorithm}
\caption{Prohibition norm acquisition}\label{alg:prohibition_acquisition}
\SetKwFunction{AddPlan}{.add\_plan}
\SetKwComment{Comment}{$\triangleright$ }{}
\KwIn{Norm=$prohibition(Action, Parameters)$}
\KwOut{new plans to enable norm compliance added to plan list}

add belief $prohibition(Action, Parameters)$\;
acquire list $relevantPlansAffected$ %\Comment*[r]{Check Algorithm \ref{alg:relevant_plans_modification}}
refine $relevantPlansAffected$ %\Comment*[r]{Check Algorithm \ref{alg:relevant_plans_refinement}}
remove the relevant plans from the plan list\;
create list $normativePlans$ %\Comment*[r]{Check Algorithm \ref{alg:create_new_normative_plans}}
\lForEach{plan $p$ on $normativePlans$}{\AddPlan{p}}
\end{algorithm}

\begin{algorithm}
\caption{Relevant plans acquisition and modification (Java)}\label{alg:relevant_plans_modification}
\SetKwFunction{RelevantPlans}{.relevant\_plans}
\KwData{$Action$ and list of $Parameters$}
\KwResult{Jason Trigger with format similar to $Action(\_)$ usable with the \RelevantPlans internal action}
\eIf{$Parameters$ is atomic}{
    $terms$ = '\_'\;
}{\If{$Parameters$ is List}{
    \lForEach{Parameter $p$ on $Parameters$}{$terms$ += '\_'}
 }
}
return trigger $Action$($terms$)\;
\end{algorithm}

\begin{algorithm}
\caption{Relevant plan list refinement using Parameters (Java)}\label{alg:relevant_plans_refinement}
\KwData{$planList$ as args[0], $labelList$ as args[1], $parameters$ as args[2]}
\KwResult{$planList$ and $labelList$ with plans and labels that contains $parameters$}
\ForEach{plan p on $planList$}{
    \If{$p$ contains $parameters$}{
        $planList$.remove($p$)\;
        $labelList$.remove($p$)\;
    }
}
return $planList$, $labelList$\;
\end{algorithm}

\begin{algorithm}
\caption{Prohibition plan creation (Java)}\label{alg:create_new_normative_plans}
\KwData{$planList$ as args[0]}
\KwResult{$planList$ with new normative aware prohibition plans}
\SetKwComment{Comment}{// }{ }
\ForEach{plan $p$ on $planList$}{
    pattern = ``(\_[0-9]*)"\;
    i = 1\;
    stringNewTerms = ``"\;
    HashMap$<$Term, Term$>$ newTerms = new HashMap$<>$();
    \Comment{If the plan is generic it might contain anonymous variables, representend by an underscore in Jason. We need to replace them with a new variable with a workable syntax}
    \ForEach{$term$ in $p$}{
        \eIf{$pattern$ matches $term$}{
            newTerms.put($pattern$, new StringTermImpl(``Param"+i))\;
            stringNewTerms += ``Param"+i\;
            i++\;
        }{
            stringNewTerms += $t$\;
        }
    }
    triggerAction = $plan$.name \Comment*[l]{$plan$ functor}
    newTrigger = new Trigger(TEOperator.add, TEType.achieve, triggerAction+stringNewTerms) \Comment*[l]{The header of the new plans}
}
\end{algorithm}

{
\setlength{\interspacetitleruled}{-.4pt}%
\begin{algorithm}
\setcounter{AlgoLine}{12}
\SetKwComment{Comment}{// }{ }
%This is to hide Begin keyword
\SetKwBlock{Begin}{}{end} 
\TitleOfAlgo{Continuation (1) of Algorithm \ref{alg:create_new_normative_plans}}
\Begin{
    \Comment{1. Modify the original plan to point that it should work if the prohibition is not established, i.e. the action is allowed}
	\Comment{1.1. Create the new label}
	annots.add(``normative")\;
	annots.add(``not\_prohibition")\;
	newLabel.addAnnots(annots)\;
	\Comment{1.2 Create the new logical formula}
	planContext = plan.getContext()\;
	String triggerTerms = stringNewTerms.values().toString().replace("\"", "")\;
    \eIf{planContext == null}
    {
    	newContext = ``not prohibition("+triggerAction+``, " + triggerTerms + ``)"\;
    }
    {
    	newContext = planContext.toString() + `` \& not prohibition("+triggerAction+``, " + triggerTerms + ")"\;
    }
	newLogicalFormula = newContext\;
	\Comment{1.3. Loop over the new body and update it back properly using the HashMap}
	newPlanBody = ``"\;
	\While{planBody.getBodyNext() != null}{
	    Check if the line contains a word stored in $newTerms$ and replace it \;
	    planBody = planBody.getBodyNext();
    }
	\Comment{1.4. Form final plan}
	Plan notProhibitionPlan = new Plan(newLabel, newTrigger, newLogicalFormula, planBody)\;     
}
\end{algorithm}
}

{
\setlength{\interspacetitleruled}{-.4pt}%
\begin{algorithm}
\setcounter{AlgoLine}{27}
\SetKwComment{Comment}{// }{ }
%This is to hide Begin keyword
\SetKwBlock{Begin}{}{end} 
\TitleOfAlgo{Continuation (2) of Algorithm \ref{alg:create_new_normative_plans}}
\Begin{
    \Comment{2. Insert the new plan}
    \Comment{2.1}
    \Comment{2.2}
    \Comment{2.3}
    \Comment{3. }
    
    // 2. Insert the new plan
	// 2.1.
	String namespace2 = planLabel.getFunctor() + "2";
	ListTerm annots2 = planLabel.getAnnots().cloneLT();
	Atom aNormative2 = new Atom("normative");
	Atom aProhibition2 = new Atom("prohibition");
	annots2.add(aNormative2);
	annots2.add(aProhibition2);
	newLabel = new Pred(namespace2);
	newLabel.addAnnots(annots2);

	// 2.2.
	//triggerTerms = "[Param1]";
	if (planContext == null)
		newContext = "prohibition(publish, " + triggerTerms + ")";
	else
		newContext = planContext.toString() + " \& prohibition(publish, " + triggerTerms + ")";
	newLogicalFormula = LogExpr.parseExpr(newContext);

	// 2.3.
	// Term t = new Structure(".print(\"I cannot do this action\")");
	PlanBody newEmptyBody = new PlanBodyImpl(BodyType.none);
	//TODO: Cambiar t por planTrigger
	Plan prohibitionPlan = new Plan(newLabel, newTrigger, newLogicalFormula, newEmptyBody);

	// 3. We add the new plans to the results
	resultList.add(notProhibitionPlan);
	resultList.add(prohibitionPlan);
}
\end{algorithm}
}
\end{comment}
